Sparse MTTKRP Acceleration for Tensor Decomposition on GPU

Sparse Matricized Tensor Times Khatri-Rao Product (spMTTKRP) is the bottleneck kernel of sparse tensor decomposition. In this work, we propose a GPU-based algorithm design to address the key challenges in accelerating spMTTKRP computation, including (1) eliminating global atomic operations across GPU thread blocks, (2) avoiding the intermediate values being communicated between GPU thread blocks and GPU global memory, and (3) ensuring a balanced distribution of workloads across GPU thread blocks. Our approach also supports dynamic tensor remapping, enabling the above optimizations in all the modes of the input tensor. Our approach achieves a geometric mean speedup of 1.5x, 2.0x, and 21.7x in total execution time across widely used datasets compared with the state-of-the-art GPU implementations. Our work is the only GPU implementation that can support tensors with modes greater than 4 since the state-of-the-art works have implementation constraints for tensors with a large number of modes.

==> content/5_composer.tex <==
\section{System Composer}
%  1 page
\setlength{\textfloatsep}{1.0pt plus 1.0pt minus 1.0pt}
\setlength{\floatsep}{1.0pt plus 1.0pt minus 1.0pt}
\setlength{\intextsep}{1.0pt plus 1.0pt minus 1.0pt}
\label{sec:sysconfigurator}
Given the user-specified Replay Manager (RM) and Learner metadata in the Optimizer Construction Program as inputs, 
the goals of the system composer are to (A) determine the best-performing accelerator configuration within each device for all the primitives, and (B) determine an optimal primitive-to-device assignment that maximizes system performance.
% \vspace{-1em}
\subsection{Accelerator Setup and Performance Estimation}
\label{sec:asetup}
To realize goal (A), we customize the parameterized accelerators described in Section \ref{sec:codebase} to suit the user-input RM and Learner specifications. 
% we can remove this sentence?
% Customization refers to adapting the degree of parallelism assigned to the primitive on a processor or accelerator (e.g., number of compute cores allocated on CPU or GPU, number of pipeline modules and buffer sizes allocated on FPGA).
Based on the customized accelerators, we obtain the expected latency of executing each primitive in one DRL iteration on each of the available devices, and store these latency numbers in a Primitive Device Assignment Matrix for further analysis of system performance in goal (B).

% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.5}
% \begin{table}[]
% \scriptsize
% \centering
% \caption{Primitive Device Assignment Matrix: An Example }
% \label{tab:compute-perf}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{} & \textbf{\begin{tabular}[c]{@{}c@{}}RM only\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Learner only\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RM \& Learner\end{tabular}} \\ \hline
% \textbf{CPU} & $T_{RM}(CPU)$ & $T_{Learner}(CPU)$ & $T_{RM'}$, $T_{Learner'}(CPU)$ \\ \hline
% \textbf{GPU} & $T_{RM}(GPU)$ & $T_{Learner}(GPU)$ & $T_{RM'}$, $T_{Learner'}(GPU)$ \\ \hline
% \textbf{FPGA} & $T_{RM}(FPGA)$ & $T_{Learner}(FPGA)$ & $T_{RM'}$, $T_{Learner'}(FPGA)$ \\ \hline
% \end{tabular}
% \end{table}
% \textcolor{red}{
The Primitive Device Assignment Matrix is a 3$\times N$ table. The $N$ rows denote the $N$ available devices; each column refers to either one primitive or a combination of both primitives to be assigned to one device. 
% An example of a Primitive Device Assignment Matrix for a single-node processor connected to two accelerators is shown in Table \ref{tab:compute-perf}. The notion of $T^x_y$ in the table entries denotes the latency of performing one iteration of the given primitive $x$ on device $y$ (For the RM, the latencies include those of the sampling, updates and insertions). 
Each entry $T^x_y$ in the table denotes the latency of performing one iteration of a given primitive (or a combination of 2 primitives) $x$ on device $y$ (For RM, the latency includes times of the sampling, updates and insertions). 
% }
We explain how the table entries are populated based on accelerator setups as follows: 

\textit{Primitive Setup on a CPU/GPU :} 
% For the Learner, we allocate threads for training such that the time for processing $BS$ experiences matches that of generating $BS$ experiences by the Actors. 
% For the RM, the degree of parallelism $W$ is ($\text{Total \# threads in the CPU - \# threads for the Actors}$), clipped by the range $[1,BS]$. 
For the primitives that can be mapped to the CPU, i.e., RM and Actors, we allocate their number of threads initially based on the ratio of their single-iteration latency for processing/producing one experience in order to match their throughput.
Note that based on this setup, if RM ends up being mapped to an accelerator that provide faster RM processing, the Actors will be initially set to occupy all available threads, and will be further dynamically adjusted based on the runtime data processing speed of Actors and Learner (Section \ref{sec:runtime-res}).
% \textcolor{green}{TODO: actor}
% Afterward, we run the primitive with synthetic data for $1K$ iterations and profile the per-iteration latency and power consumption for filling the $T(CPU)$ entries in the Primitive Device Assignment Matrix.
%\textit{Acceleration Setup on a GPU:}  
For the RM on a GPU, the degree of parallelism is set to $BS$.
The sum tree is stored in the GPU global memory.
For the Learner on a GPU, we search for the best-performing number of streams in the range $[1,BS]$ by recording their per-SGD-step latencies. 
% Afterward, we use the optimal latency and power consumption of each primitive for filling the Primitive Device Assignment Matrix.

\textit{Accelerator Configuration on an FPGA:} 
The RM and the Learner can both be mapped to the same FPGA device only if the total buffer size required by the RM and Learner modules is smaller than the total amount of SRAM resources. This is to avoid efficiency losses in accesses to off-chip memory. For the RM, the number of Autorun kernels in the pipeline is configured to match the tree depth, and the buffer sizes are configured based on their corresponding tree levels. For the Learner, the number of pipelines $DP$ is set to the largest value within resource capacity.
The amount of compute resources allocated to each pipeline stage, $UF$, is tuned such that all pipeline stages are load balanced (for the maximal effective hardware utilization): 
% \begin{multline}
% \small
%     T_{stage}=\frac{\# MAC^{\text{FP L}_1}}{UF^{\text{FP L}_1}} =
%     % \frac{\# MACC^\text{FP L2}}{UF^\text{FP L2}} 
%     ... =\frac{\# MAC^{\text{GA L}_N}}{UF^{\text{FP L}_N}};\\
% \small
%     \text{where }UF^{\text{FP L}_1}+UF^{\text{FP L}_2}+...+UF^{\text{FP L}_N}\leq \frac{\text{\#DSPs}}{DP}.
% \end{multline}
\begin{equation}
    T_{stage}=\frac{\# MAC^{\text{FP L}_1}}{UF^{\text{FP L}_1}} =
    % \frac{\# MACC^\text{FP L2}}{UF^\text{FP L2}} 
    ... =\frac{\# MAC^{\text{GA L}_N}}{UF^{\text{FP L}_N}}; \text{where }\sum UF\leq \frac{\text{\#DSPs}}{DP}.
\end{equation}
We obtain the latency of accelerators on FPGA through performance modeling:
\begin{gather}
% \vspace{-4pt}
    T_{RM}^\text{sampling}=2\times F\times (BS+D)+T_{comm}^{(i\rightarrow FPGA)}\\
    T_{RM}^\text{update or insert}=2\times (BS+D)+T_{comm}^{(i\rightarrow FPGA)}\\
    T_{Learner}=T_{stage}\times (BS+3\times(\text{\#layers}-1))
    % \vspace{-4pt}
\end{gather}
In equations 3-5, the pipeline latencies are calculated 
% using the following steps: First, we determine the per-stage latency. Next, we multiply this per-stage latency by the sum of batch size $BS$ and pipeline overhead $D$, where $D$ is the pipeline fill/drain overhead
by multiplying single pipeline stage latency by the batch size $BS$ and pipeline fill/drain overhead $D$ ($D$ equals the sum tree depth in RM and \# layer propagation's in Learner, respectivaly).
% ($D$ is directly proportional to the depth of the pipeline). 
% In the Replay Manager (RM), $D$ equals the sum tree depth, while in the Learner, it equals the total number of layer propagations.
$T_{comm}$ refers to the communication time of taking inputs from device $i$ executing other primitives.
% residing on the same or different device, 
% which 
% can be modeled as $lat+\frac{\text{data size}}{\text{bandwidth}}$. The data transfer latency overhead ($lat$) and bandwidth characteristics will be 
They are filled in Algorithm \ref{algo:mapping} - Equation \ref{eq:obj} depending on whether the communication is within the same device (e.g., through DDR) or across different devices (e.g., through PCIe). 
% In Equation 4, $i$ refers to the device that initiates sampling. In Equation 5, $i$ refers to either the Actors device (CPU) for insertion requests or the Learner device for update requests.
\vspace{-5pt}
\subsection{Heterogeneous System Composition}
\label{sec:mapping}
% \begin{algorithm}[!t]
\begin{algorithm}
\small
    \caption{Heterogeneous System Composition Algorithm}
    \label{algo:mapping}
    \begin{algorithmic}[1]
        \STATE {\bfseries Input:} Primitive Device Assignment Matrix $M$, 
        \STATE \texttt{\# Step 1: Primitive Placement}
        \STATE D[{\text{RM}}], $D[{\text{Learner}}]=argmax_{i,j}\{\frac{\text{Iteration Batch Size}}{T_\text{itr}}\}$
        \STATE where $i,j$ denotes available devices for RM and Learner in $M$,
        \begin{equation}
        \small
        \label{eq:obj}
        T_{\text {itr}}=\eqnmark{comm1}{T_{RM}^{\text {sampling}}(i)}+\max (\eqnmark{comm3}{T_{R M}^{\text {insert}}(i)}, \eqnmark{comm2}{T_{RM}^{\text{update}}(i)}+T_{\text {Learner}}(j))
        \end{equation}
\annotate[yshift=0.5em]{below,right}{comm1}{$T_{\text {comm}}^{(i \rightarrow j)}$}
\annotate[yshift=0.5em]{below,right}{comm2}{$T_{\text{comm}}^{(j \rightarrow i)}$}
\annotate[yshift=0.5em]{below,right}{comm3}{$T_{\text {comm }}^{(cpu \rightarrow i)}$}
        \STATE \textbf{Output} $D[\text{Learner}], D[\text{RM}]$
        % \STATE
        \STATE \texttt{\# Step 2: Memory Component Placement}
        \STATE Initialize $D[\text{Exp Memory}]$; min$\_$traffic$\leftarrow \infty$
        \STATE $C_{\text{Learner}}\leftarrow BS\times (E+1)$; $C_{\text{Actor}}\leftarrow N_{Actor}\times E$; $C_{\text{RM}}\leftarrow BS$ 
        \FOR{$i$ in [Learner, Actors, RM]} 
         \STATE Total data traffic = $\sum^{i'\in\{\text{Learner,Actors,RM}\}} \frac{C_{i'}}{\text{bandwidth}(D[i],D[i'])}$
         \IF{Total data traffic $<$ min$\_$traffic}
         % \STATE min$\_$traffic $\leftarrow$ min(Total data traffic, min$\_$traffic);  
         \STATE min$\_$traffic $\leftarrow$ Total data traffic; $D[\text{Exp Memory}]\leftarrow D[i]$;
         % \STATE $D[\text{Exp Memory}]\leftarrow D[i]$
         \ENDIF
        \ENDFOR
        \STATE \textbf{Output} $D[\text{Exp Memory}]$
    \end{algorithmic}
\end{algorithm}
Based on a completed Primitive Device Assignment Matrix, we develop a Heterogeneous System Composition Algorithm (Algorithm \ref{algo:mapping}).
It first determines the best device assignment of the primitives to maximize achievable compute throughput,
then places the memory component (Exp Memory) to minimize the total data traffic.

% \vspace{-1em}
In Step 1 (lines 2-5, Algorithm \ref{algo:mapping}), the training throughput can be estimated using the processed batch size in each iteration, $BS$, and the iteration execution time, $T_{itr}$. $T_{itr}$ is defined in Equation \ref{eq:obj}. 
The critical path in an iteration is the priority sampling followed by SGD training and priority update, while the other replay operations overlap with the training process. 
The required costs of communication with other compute modules are encapsulated in each component of Equation \ref{eq:obj} corresponding to the candidate devices $i,j$ for RM and Learner, where $i,j$ are permutated to include all the device assignment choices. When $i=j$, the latencies are sampled from the third column of the Compute-Performance Table.
% (e.g., Table \ref{tab:compute-perf}). 
The complexity of Step 1 is $O(N^2)$, given $N$ available devices on the heterogeneous platform.
% $O(P(N,2))=O(\frac{N!}{(N-2)!})$.
In Step 2 (lines 7-13, Algorithm \ref{algo:mapping}), we decide on the device assignment of the Exp Memory. The data traffic wrt the Exp Memory during each iteration includes $BS$ words of sampling indices from the $D_\text{Learner}$, $BS\times E$ sampled experiences to the $D_\text{Learner}$ (where $E$ is the size of each experience for the given benchmark), and $N_{Actor}\times E$ inserted experiences from the Actors. These communication costs are denoted as $C$ in Algorithm \ref{algo:mapping}. We place Exp Memory on the device that minimizes the total data traffic based on available bandwidths between devices (e.g., PCIe) and within each device (e.g., DDR). The complexity of Step 2 is $O(1)$, as the number of primitives is constant.


